A global perspective to connections on principal 2-bundles

For a strict Lie 2-group, we develop a notion of Lie 2-algebra-valued differential forms on Lie groupoids, furnishing a differential graded-commutative Lie algebra equipped with an adjoint action of the Lie 2-group and a pullback operation along Morita equivalences between Lie groupoids. Using this notion, we define connections on principal 2-bundles as Lie 2-algebra-valued 1-forms on the total space Lie groupoid of the 2-bundle, satisfying a condition in complete analogy to connections on ordinary principal bundles. We carefully treat various notions of curvature, and prove a classification result by the non-abelian differential cohomology of Breen-Messing. This provides a consistent, global perspective to higher gauge theory.

==> kobib.tex <==
\makeatletter

\def\kobiburl#1{
   \IfBeginWith
     {#1}
     {http://arxiv.org/abs/}
     {\kobibarxiv{#1}}
     {\kobiblink{#1}}}
\def\kobibarxiv#1{\href{#1}{\texttt{[arxiv:\StrGobbleLeft{#1}{21}]}}}
\def\kobiblink#1{
  \StrSubstitute{#1}{\~{}}{\string~}[\myurl]
  \StrSubstitute{#1}{_}{\underline{\;\;}}[\mylink]
  \StrSubstitute{\mylink}{&}{\&}[\mylink]
  \StrSubstitute{\mylink}{/}{/\allowbreak}[\mylink]
  \newline Available as: \mbox{\;}
  \href{\myurl}{\texttt{\mylink}}}

\def\noarxiv{\def\kobibarxiv##1{}}
\def\nolinks{\def\kobiblink##1{}}

\renewenvironment{thebibliography}[1]
     {\ifx\relax#1\relax\else
      \tocsection{\refname}
      \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}%
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m
      \fi}

\makeatother




==> theorems.tex <==
\makeatletter

\def\setsecnumdepth#1{
  \setcounter{secnumdepth}{#1}
  \setcounter{equation}{0}
  \setcounter{theorem}{0}
  \ifnum\c@secnumdepth=0
    \def\theequation{\arabic{equation}}    
    \def\thetheorem{\arabic{theorem}}    
    \def\theproposition{\arabic{proposition}}    
    \def\thecorollary{\arabic{corollary}}    
    \def\thedefinition{\arabic{definition}}    
    \def\theconstruction{\arabic{construction}}    
    \def\thelemma{\arabic{lemma}}    
    \def\theremark{\arabic{remark}}    
    \def\theproblem{\arabic{problem}}    
    \def\theexample{\arabic{example}}    
    \def\theexercise{\arabic{exercise}}    
  \fi
  \ifnum\c@secnumdepth=1
    \numberwithin{equation}{section}
    \@addtoreset{theorem}{section}
    \def\theequation{\thesection.\arabic{equation}}    
    \def\thetheorem{\thesection.\arabic{theorem}}    
    \def\theproposition{\thesection.\arabic{proposition}}    
    \def\thecorollary{\thesection.\arabic{corollary}}    
    \def\thedefinition{\thesection.\arabic{definition}}    
    \def\theconstruction{\thesection.\arabic{construction}}    
    \def\thelemma{\thesection.\arabic{lemma}}    
    \def\theremark{\thesection.\arabic{remark}}    
    \def\theproblem{\thesection.\arabic{problem}}    
    \def\theexample{\thesection.\arabic{example}}    
    \def\theexercise{\thesection.\arabic{exercise}}    
  \fi
  \ifnum\c@secnumdepth=2
    \numberwithin{equation}{subsection}
    \@addtoreset{theorem}{subsection}
    \def\theequation{\thesubsection.\arabic{equation}}    
    \def\thetheorem{\thesubsection.\arabic{theorem}}    
    \def\theproposition{\thesubsection.\arabic{proposition}}    
    \def\thecorollary{\thesubsection.\arabic{corollary}}    
    \def\thedefinition{\thesubsection.\arabic{definition}}    
    \def\theconstruction{\thesubsection.\arabic{construction}}    
    \def\thelemma{\thesubsection.\arabic{lemma}}    
    \def\theremark{\thesubsection.\arabic{remark}}    
    \def\theproblem{\thesubsection.\arabic{problem}}    
    \def\theexample{\thesubsection.\arabic{example}}    
    \def\theexercise{\thesubsection.\arabic{exercise}}    
  \fi  
  \ifnum\c@secnumdepth>2
    \numberwithin{equation}{subsubsection}
    \@addtoreset{theorem}{subsubsection}
    \def\theequation{\thesubsubsection.\arabic{equation}}    
    \def\thetheorem{\thesubsubsection.\arabic{theorem}}    
    \def\theproposition{\thesubsubsection.\arabic{proposition}}    
    \def\thecorollary{\thesubsubsection.\arabic{corollary}}    
    \def\thedefinition{\thesubsubsection.\arabic{definition}}    
    \def\theconstruction{\thesubsubsection.\arabic{construction}}    
    \def\thelemma{\thesubsubsection.\arabic{lemma}}    
    \def\theremark{\thesubsubsection.\arabic{remark}}    
    \def\theproblem{\thesubsubsection.\arabic{problem}}    
    \def\theexample{\thesubsubsection.\arabic{example}}    
    \def\theexercise{\thesubsubsection.\arabic{exercise}}    
  \fi  
}

%%% Theoreme definieren

\newlength{\theoremspace}
\setlength{\theoremspace}{1em}

\newtheoremstyle{theorem}{\theoremspace}{\theoremspace}{\normalfont\itshape}{0pt}{\normalfont\bfseries}{.}{ }{\thmname{#1}\space\thmnumber{#2}\thmnote{ (#3)}}
\newtheoremstyle{remark} {\theoremspace}{\theoremspace}{\normalfont}        {0pt}{\normalfont\itshape} {.}{ }{\thmname{#1}\space\thmnumber{#2}\thmnote{ (#3)}}

\declaretheorem[style=theorem,name=\nameTheorem]{theorem}
\declaretheorem[style=theorem,name=\nameProposition,sibling=theorem]{proposition}
\declaretheorem[style=theorem,name=\nameCorollary,sibling=theorem]{corollary}
\declaretheorem[style=theorem,name=\nameDefinition,sibling=theorem]{definition}
\declaretheorem[style=theorem,name=\nameLemma,sibling=theorem]{lemma}

\declaretheorem[style=theorem,name=\nameTheorem]{maintheorem}
\declaretheorem[style=theorem,name=\nameProposition,sibling=maintheorem]{mainproposition}
\declaretheorem[style=theorem,name=\nameCorollary,sibling=maintheorem]{maincorollary}
\declaretheorem[style=theorem,name=\nameDefinition,sibling=maintheorem]{maindefinition}

\declaretheorem[style=remark,name=\nameRemark,sibling=theorem]{remark}
\declaretheorem[style=remark,name=\nameConstruction,sibling=theorem]{construction}
\declaretheorem[style=remark,name=\nameProblem,sibling=theorem]{problem}
\declaretheorem[style=remark,name=\nameExample,sibling=theorem]{example}
\declaretheorem[style=remark,name=\nameExercise,sibling=theorem]{exercise}

%%% Cref konfiguieren

\crefname{theorem}{\nameTheorem}{\nameTheorems}
\crefname{maintheorem}{\nameTheorem}{\nameTheorems}
\crefname{definition}{\nameDefinition}{\nameDefinitions}
\crefname{construction}{\nameConstruction}{\nameConstructions}
\crefname{corollary}{\nameCorollary}{\nameCorollaries}
\crefname{proposition}{\nameProposition}{\namePropositions}
\crefname{lemma}{\nameLemma}{\nameLemmas}
\crefname{remark}{\nameRemark}{\nameRemarks}
\crefname{problem}{\nameProblem}{\nameProblems}
\crefname{example}{\nameExample}{\nameExamples}
\crefname{exercise}{\nameExercise}{\nameExercises}

\crefname{section}{\nameSection}{\nameSections}
\crefname{appendix}{\nameAppendix}{\nameAppendixs}
\crefname{enumi}{\unskip}{\unskip}
\crefname{equation}{\nameEquation}{\nameEquations}

\crefname{}{}{}
\crefformat{}{#2#1#3}


%%% Parentlabel belegen

\def\@parenttype{}
\def\@parentcounter{}

\addtotheorempostheadhook{%
  \protected@edef\@parenttype{\@currenvir}%
  \protected@edef\@parentcounter{\@currentlabel}%
}

%%% Liste nur in neuer Zeile beginnen

\addtotheorempostheadhook{\leavevmode}

%%%% Verweise auf Enumerate %%%%

\def\clabel#1{%
  % Label für Bakoma \cref{*}
  \protected@edef\@currentlabel{\csname label\@enumctr\endcsname}%
  \cref@old@label{#1*}% 
  %
  % Label für Bakoma \cref{}
  \protected@edef\@currentlabel{\@parentcounter\space\csname label\@enumctr\endcsname}%
  \cref@old@label{#1}
  %
  % Label für MikTeX \cref{*}
  \protected@edef\@currentlabel{[enumi][\arabic{enumi}][]\csname label\@enumctr\endcsname}%
  \@bsphack
  \protected@write\@auxout{}%
         {\string\newlabel{#1*@cref}{{\@currentlabel}{\thepage}}}%
  \@esphack
  %  
  % Label für MikTeX \cref{}
  \protected@edef\@currentlabel{[\@parenttype][\arabic{enumi}][]\@parentcounter\space\csname label\@enumctr\endcsname}%
  \@bsphack
  \protected@write\@auxout{}%
         {\string\newlabel{#1@cref}{{\@currentlabel}{\thepage}}}%
  \@esphack
  }

\AtBeginDocument{%
  \let\@oldlabel\label%
  \def\label#1{\def\@tempa{enumerate}\ifx\@tempa\@currenvir\clabel{#1}\else\@oldlabel{#1}\fi}}


%%% Folgendes sind gekürzte Originaldefinitionen von cleveref, ohne die \namecref in Bakoma nicht funktionieren. 
%%% Wenn man sie hier wiederholt, funktionieren sie, dafür kompiliert MikTex nicht mehr. 

%\def\namecref#1{\@setnamecref{cref}{#1}{}{}}
%\def\@setnamecref#1#2#3#4{%
%  \cref@gettype{#2}{\@tempa}%
%  \edef\@tempa{\expandafter\noexpand\csname #1@\@tempa @name#3\endcsname}%
%  \expandafter\@@setnamecref\expandafter{\@tempa}{#4}%
%}%


\makeatother
